Is the cluster environment quenching the Seyfert activity in elliptical and spiral galaxies?

We developed a hierarchical Bayesian model (HBM) to investigate how the presence of Seyfert activity relates to their environment, herein represented by the galaxy cluster mass, $M_{200}$, and the normalized cluster-centric distance, $r/r_{200}$. We achieved this by constructing an unbiased sample of galaxies from the Sloan Digital Sky Survey, with morphological classifications provided by the Galaxy Zoo Project. A propensity score matching approach is introduced to control for the effects of confounding variables: stellar mass, galaxy colour, and star formation rate. The connection between Seyfert-activity and environmental properties in the de-biased sample is modelled within an HBM framework using the so-called logistic regression technique, suitable for the analysis of binary data (e.g., whether or not a galaxy hosts an AGN). Unlike standard ordinary least square fitting methods, our methodology naturally allows modelling the probability of Seyfert-AGN activity in galaxies on their natural scale, i.e. as a binary variable. Furthermore, we demonstrate how an HBM can incorporate information of each particular galaxy morphological type in a unified framework. In elliptical galaxies, our analysis indicates a strong correlation of Seyfert-AGN activity with $r/r_{200}$, and a weaker correlation with the mass of the host. In spiral galaxies these trends do not appear, suggesting that the link between Seyfert activity and the properties of spiral galaxies are independent of the environment.

==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 3.61 (2015/06/12)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.61}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcb@segment@state=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcol@frame,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcol@back,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcol@backtitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcol@frame,bottom color=tcbcol@back,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcol@frame}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@backtitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcol@frame}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcol@backlower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}


\tikzset{beamer@color/.style={top color=tcbcol@back,bottom color=tcbcol@back!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcb@segment@state
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}


\tcbset{%
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.store in=\kvtcb@style@boxedtitle,%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \colorlet{tcbtranscol@frame}{tcbcol@frame}%
      \colorlet{tcbtranscol@back}{tcbcol@backtitle}%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@boxedtitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[colframe=tcbtranscol@frame,colback=tcbtranscol@back,size=title,code={\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}}\endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}};
  }},
  fill plain picture/.style={path picture={%
    \tcb@set@waterbox@to@picture{#1}%
    \node at (path picture bounding box.center) {\box\tcb@waterbox};
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]{#1}};
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcol@frame,bottom color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  title style={left color=tcbcol@frame,right color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options]}%
      \tcb@temp{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}[underlay={%
        \begin{tcbclipinterior}%
        \edef\tcb@temp{\noexpand\tikzset{fill image options={\expandonce\kvtcb@graphics@options}}}%
        \tcb@temp%
        \path[fill zoom image={\imagepath}]
          ([xshift=\kvtcb@boxsep+\kvtcb@leftupper,yshift=\kvtcb@boxsep+\kvtcb@bottom]interior.south west) rectangle
          ([xshift=-\kvtcb@boxsep-\kvtcb@rightupper,yshift=-\kvtcb@boxsep-\kvtcb@top]interior.north east);
        \end{tcbclipinterior}%
        }]%
      \end{tcolorbox}%
    \else%
      \begin{tcolorbox}%
        \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth]}%
        \tcb@temp{\imagepath}%
      \end{tcolorbox}%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
}


\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcol@back!85!tcbcol@frame,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title style=,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 3.61 (2015/06/12)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2014 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.61}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.61 (2015/06/12)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2014 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.61}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1:#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5:##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,%
  },
  initialize@reset=reset@theorems,
}


